Blizzard: Adding True Persistence to Main Memory Data Structures

Persistent memory (PMEM) devices present an opportunity to retain the flexibility of main memory data structures and algorithms, but augment them with reliability and persistence. The challenge in doing this is to combine replication (for reliability) and failure atomicity (for persistence) with concurrency (for fully utilizing persistent memory bandwidth). These requirements are at odds due to the sequential nature of replicating a log of updates versus concurrent updates that are necessary for fully leveraging the path from CPU to memory. We present Blizzard -- a fault-tolerant, PMEM-optimized persistent programming runtime. Blizzard addresses the fundamental tradeoff by combining (1) a coupled operations log that permits tight integration of a PMEM-specialized user-level replication stack with a PMEM-based persistence stack, and (2) explicit control over the commutativity among concurrent operations. We demonstrate the generality and potential of Blizzard with three illustrative applications with very different data structure requirements for their persistent state. These use cases demonstrate that with Blizzard, PMEM native data structures can deliver up to 3.6x performance benefit over the alternative purpose-build persistent application runtimes, while being simpler and safer (by providing failure atomicity and replication).

==> Makefile <==
PAPER=paper
TARGET=paper


paper:
	pdflatex $(PAPER).tex < /dev/null
	bibtex $(PAPER)
	pdflatex $(PAPER).tex < /dev/null
	pdflatex $(PAPER).tex </dev/null

clean:
	rm -f *.aux *.log *.out *.bbl *.blg *~ *.bak $(TARGET).ps $(TARGET).pdf

# Check spelling with aspell
spellcheck:
	find . -name "*.tex" -exec aspell --lang=en --mode=tex --dont-suggest --personal=./.aspell.en.pws check "{}" \;

